Semantics of Attack-Defense Trees for Dynamic Countermeasures and a New Hierarchy of Star-free Languages

We present a mathematical setting for attack-defense trees, a classic graphical model to specify attacks and countermeasures. We equip attack-defense trees with (trace) language semantics allowing to have an original dynamic interpretation of countermeasures. Interestingly, the expressiveness of attack-defense trees coincides with star-free languages, and the nested countermeasures impact the expressiveness of attack-defense trees. With an adequate notion of countermeasure-depth, we exhibit a strict hierarchy of the star-free languages that does not coincides with the classic one. Additionally, driven by the use of attack-defense trees in practice, we address the decision problems of trace membership and of non-emptiness, and study their computational complexities parameterized by the countermeasure-depth.

==> adtfigures.tex <==
%% to draw 
\makeatletter
\newcommand{\arc}[5]{%
  \pgfsetlinewidth{1.4pt}%
  \newdimen\a\newdimen\b%
  \pgf@process{\pgfpointanchor{#1}{center}}%
  \pgf@xa=\pgf@x\pgf@ya=\pgf@y%
  \pgf@process{\pgfpointdiff{\pgfpointanchor{#1}{east}}{\pgfpointanchor{#1}{center}}}%
  \advance\pgf@x by -8pt\relax \a=\pgf@x%
  \pgf@process{\pgfpointdiff{\pgfpointanchor{#1}{south}}{\pgfpointanchor{#1}{center}}}%
  \advance\pgf@y by 8pt\relax\b=\pgf@y\relax%
  \pgfkeys{/pgf/fpu, /pgf/fpu/output format=fixed}
  \pgf@process{\pgfpointdiff{\pgfpointanchor{#3}{center}}{\pgfpointanchor{#1}{center}}}%
  \pgfmathsetlengthmacro\rightx{\a*\b/sqrt(\a*\a*\pgf@y*\pgf@y + %
      \b*\b*\pgf@x*\pgf@x)*\pgf@x + \pgf@xa}%
  \pgfmathsetlengthmacro\righty{\a*\b/sqrt(\a*\a*\pgf@y*\pgf@y + %
    \b*\b*\pgf@x*\pgf@x)*\pgf@y + \pgf@ya}%
  \pgf@process{\pgfpointdiff{\pgfpointanchor{#2}{center}}{\pgfpointanchor{#1}{center}}}%
  \pgfmathparse{atan((-\a/\b)*(\righty - \pgf@ya)/(\rightx - \pgf@xa))}%
  \pgfmathsetmacro\rightAngle{\pgfmathresult>0?360-\pgfmathresult:180-\pgfmathresult}%
  \pgfmathsetmacro\leftAngle{360-atan((-\a/\b)*(\a*\b/sqrt(\a*\a*\pgf@y*\pgf@y + %
    \b*\b*\pgf@x*\pgf@x)*\pgf@y)/(\a*\b/sqrt(\a*\a*\pgf@y*\pgf@y + %
      \b*\b*\pgf@x*\pgf@x)*\pgf@x))}%
  \pgfkeys{/pgf/fpu=false}%
  \pgfmoveto{\pgfpoint{\rightx}{\righty}}%
  \ifstrequal{#4}{t}{\pgfsetarrowsstart{angle 90}}{\pgfsetarrowsstart{}}%
  \ifstrequal{#5}{d}{\pgfsetdash{{1pt}{1pt}}{0pt}}{\pgfsetdash{}{0pt}}%
  \pgfpatharc{\rightAngle}{\leftAngle}{\a and \b}\pgfusepath{draw}%
  \pgfusepath{draw}%
}
\def\andC{\arc{node@\forestove{id}}{node@\forestove{@first}}%
  {node@\pgfkeysvalueof{/forest/@node/\forestove{@last}/@previous}}{o}{s}}
\def\andN{\arc{node@\forestove{id}}%
  {node@\forestove{@first}}{node@\forestove{@last}}{o}{s}}
\def\sandN{\arc{node@\forestove{id}}%
  {node@\forestove{@first}}{node@\forestove{@last}}{t}{s}}
\def\sandC{\arc{node@\forestove{id}}{node@\forestove{@first}}%
  {node@\pgfkeysvalueof{/forest/@node/\forestove{@last}/@previous}}{t}{s}}
\def\coN{\arc{node@\forestove{id}}%
  {node@\forestove{@first}}{node@\forestove{@last}}{o}{d}}
\def\coC{\arc{node@\forestove{id}}{node@\forestove{@first}}%
  {node@\pgfkeysvalueof{/forest/@node/\forestove{@last}/@previous}}{t}{d}}



\def\inheritall#1{
  \foreach \anchor in {north,north west,north east,center,west,east,mid,center,
    mid west,mid east,base,base west,base east,south,south west,south east}{%
    \inheritanchor[from=#1]{\anchor}}%
  \inheritanchorborder[from=#1]
  \inheritbackgroundpath[from=#1]
}

\pgfdeclareshape{attacker}{
    \inheritsavedanchors[from=ellipse]
    \savedanchor\radius{%
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by.5\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y by\pgf@yb%
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@x by\pgf@xb%
    \pgf@x=1.4142136\pgf@x%
    \pgf@y=1.4142136\pgf@y%
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@y<.5\pgf@yc\pgf@y=.5\pgf@yc\fi%
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgf@x<.5\pgf@xc\pgf@x=.5\pgf@xc\fi%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \advance\pgf@x by\pgf@xb%
    \advance\pgf@y by\pgf@yb%
    \ifdim\pgf@x<\pgf@y\pgf@x=\pgf@y\fi
  }
  \inheritall{ellipse}
}
\let\forest@compute@node@boundary@attacker\forest@compute@node@boundary@circle

\def\squarecorner#1{
    \pgf@x=\the\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@x by 2\pgf@xc%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgf@x<\pgf@xb \pgf@x=\pgf@xb\fi%
    \pgf@y=\ht\pgfnodeparttextbox%
    \advance\pgf@y by\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y by 2\pgf@yc%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@y<\pgf@yb\pgf@y=\pgf@yb\fi%
    \ifdim\pgf@x<\pgf@y\pgf@x=\pgf@y\fi
    \pgf@x=1.4142136\pgf@x%
    \pgf@y=1.4142136\pgf@y%
    \pgf@x=#1.5\pgf@x%
    \advance\pgf@x by.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
    \advance\pgf@x by#1\pgf@xa%
    \pgf@y=#1.5\pgf@y%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
    \advance\pgf@y by.5\ht\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y by#1\pgf@ya%
}
\pgfdeclareshape{defender}{
    \savedanchor\northeast{\squarecorner{}}
    \savedanchor\southwest{\squarecorner{-}}
    \inheritall{rectangle}
}
\makeatother

\forestset{
  declare boolean={ispro}{false},
  common/.style={
    edge={line width=1.4pt}, line width=1.4pt, tier/.pgfmath=level(),
    l sep=10pt, align=center, s sep=30pt, anchor=center,
    on invalid={fake}{if={(ispro("!u")&&!ispro())||(!ispro("!u")&&ispro())}
      {edge={line cap=round, dash pattern=on 0pt off 4pt}}{}},
  },
  pro/.style={draw=red, attacker, ispro=true, common, inner sep=2pt},
  opp/.style={draw=green, defender,ispro=false, common, inner sep=1pt},
  noone/.style={draw, attacker, ispro=true, common, inner sep=2pt},
  oppTree/.style={for tree={opp}},
  proTree/.style={for tree={pro}},
  nooneTree/.style={for tree={noone}},
}

%% example of code

%% \begin{forest}
%% [, proTree
%%   [{$\gamma$}]
%%   [
%%     [{$\gamma$}]
%%     [
%%       [{$\gamma$}]
%%       [{$\gamma$}]
%%       [{$\gamma$}]
%%     ]\sandN
%%     ]\andN
%%     [
%%       [{$\gamma$}]
%%       [{$\gamma$}]
%%     ]\coN
%% ]
%% \end{forest}



==> forest-attwitness1.tex <==
\begin{forest}
[, nooneTree
  [{$b$}]
  [
   [${\attall[\strict{b}]}$]
   [
    [{$\etrue$}]
    [
     [{$\adtge[2]$}]
     [
      [{$\attall[a]$}]
      [{$\attall[b]$}]
     ]\andN
    ]\coN
    [{$\etrue$}]
   ]\sandN
  ]
]\coN
\end{forest}


==> forest-countermeasure.tex <==
\begin{forest}
[{Steal documents},proTree
  [{Enter building},proTree]  
  [{\begin{tabular}{c}Safe1 open\\ and\\ Safe2 open \end{tabular}}, proTree
  [{security Guard}, oppTree]
  ]
 % [{Take documents},proTree]  
%  [{Exit building},proTree]  
]\sandN
\end{forest}


==> forest-countermeasureofcountermeasure.tex <==
\begin{forest}
[, nooneTree
  [{$E$}]
  [
   [{$S_1\land S_2$}]
   [
    [{$\etrue$}]
    [
     [{$G$}]
     [{$D$}]
    ]\coN
    [{$\etrue$}]
   ]\sandN
  ]\coN
]\sandN
\end{forest}

==> forest-moreformalcountermeasure.tex <==
\begin{forest}
[, nooneTree
  [{$E$}]
  [
   [{$S_1\land S_2$}]
   [
    {$ \attall[G]$}
   ]
  ]\coN
]\sandN
\end{forest}

